CulFiT: A Fine-grained Cultural-aware LLM Training Paradigm via Multilingual Critique Data Synthesis

Large Language Models (LLMs) have demonstrated remarkable capabilities across various tasks, yet they often exhibit a specific cultural biases, neglecting the values and linguistic diversity of low-resource regions. This cultural bias not only undermines universal equality, but also risks reinforcing stereotypes and perpetuating discrimination. To address this, we propose CulFiT, a novel culturally-aware training paradigm that leverages multilingual data and fine-grained reward modeling to enhance cultural sensitivity and inclusivity. Our approach synthesizes diverse cultural-related questions, constructs critique data in culturally relevant languages, and employs fine-grained rewards to decompose cultural texts into verifiable knowledge units for interpretable evaluation. We also introduce GlobalCultureQA, a multilingual open-ended question-answering dataset designed to evaluate culturally-aware responses in a global context. Extensive experiments on three existing benchmarks and our GlobalCultureQA demonstrate that CulFiT achieves state-of-the-art open-source model performance in cultural alignment and general reasoning.

==> custom.tex <==
@article{myung2024blend,
  title={BLEnD: A Benchmark for LLMs on Everyday Knowledge in Diverse Cultures and Languages},
  author={Myung, Junho and Lee, Nayeon and Zhou, Yi and Jin, Jiho and Putri, Rifki Afina and Antypas, Dimosthenis and Borkakoty, Hsuvas and Kim, Eunsu and Perez-Almendros, Carla and Ayele, Abinew Ali and others},
  journal={arXiv preprint arXiv:2406.09948},
  year={2024}
}
@article{chiu2024culturalbench,
  title={Culturalbench: a robust, diverse and challenging benchmark on measuring the (lack of) cultural knowledge of llms},
  author={Chiu, Yu Ying and Jiang, Liwei and Lin, Bill Yuchen and Park, Chan Young and Li, Shuyue Stella and Ravi, Sahithya and Bhatia, Mehar and Antoniak, Maria and Tsvetkov, Yulia and Shwartz, Vered and others},
  journal={arXiv preprint arXiv:2410.02677},
  year={2024}
}
@article{shi2024culturebank,
  title={Culturebank: An online community-driven knowledge base towards culturally aware language technologies},
  author={Shi, Weiyan and Li, Ryan and Zhang, Yutong and Ziems, Caleb and Horesh, Raya and de Paula, Rog{\'e}rio Abreu and Yang, Diyi and others},
  journal={arXiv preprint arXiv:2404.15238},
  year={2024}
}
@inproceedings{nguyen2023extracting,
  title={Extracting cultural commonsense knowledge at scale},
  author={Nguyen, Tuan-Phong and Razniewski, Simon and Varde, Aparna and Weikum, Gerhard},
  booktitle={Proceedings of the ACM Web Conference 2023},
  pages={1907--1917},
  year={2023}
}
@article{fung2024massively,
  title={Massively multi-cultural knowledge acquisition \& lm benchmarking},
  author={Fung, Yi and Zhao, Ruining and Doo, Jae and Sun, Chenkai and Ji, Heng},
  journal={arXiv preprint arXiv:2402.09369},
  year={2024}
}
@inproceedings{liu2024multilingual,
  title={Are Multilingual LLMs Culturally-Diverse Reasoners? An Investigation into Multicultural Proverbs and Sayings},
  author={Liu, Chen and Koto, Fajri and Baldwin, Timothy and Gurevych, Iryna},
  booktitle={Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers)},
  pages={2016--2039},
  year={2024}
}
@article{shum2023automatic,
  title={Automatic prompt augmentation and selection with chain-of-thought from labeled data},
  author={Shum, KaShun and Diao, Shizhe and Zhang, Tong},
  journal={arXiv preprint arXiv:2302.12822},
  year={2023}
}
@article{rao2024normad,
  title={Normad: A benchmark for measuring the cultural adaptability of large language models},
  author={Rao, Abhinav and Yerukola, Akhila and Shah, Vishwa and Reinecke, Katharina and Sap, Maarten},
  journal={arXiv preprint arXiv:2404.12464},
  year={2024}
}
@inproceedings{huang2023culturally,
  title={Culturally aware natural language inference},
  author={Huang, Jing and Yang, Diyi},
  booktitle={Findings of the Association for Computational Linguistics: EMNLP 2023},
  pages={7591--7609},
  year={2023}
}
@inproceedings{lee2024exploring,
  title={Exploring Cross-Cultural Differences in English Hate Speech Annotations: From Dataset Construction to Analysis},
  author={Lee, Nayeon and Jung, Chani and Myung, Junho and Jin, Jiho and Camacho-Collados, Jose and Kim, Juho and Oh, Alice},
  booktitle={Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers)},
  pages={4205--4224},
  year={2024}
}
@article{achiam2023gpt,
  title={Gpt-4 technical report},
  author={Achiam, Josh and Adler, Steven and Agarwal, Sandhini and Ahmad, Lama and Akkaya, Ilge and Aleman, Florencia Leoni and Almeida, Diogo and Altenschmidt, Janko and Altman, Sam and Anadkat, Shyamal and others},
  journal={arXiv preprint arXiv:2303.08774},
  year={2023}
}
@article{wang2023not,
  title={Not all countries celebrate thanksgiving: On the cultural dominance in large language models},
  author={Wang, Wenxuan and Jiao, Wenxiang and Huang, Jingyuan and Dai, Ruyi and Huang, Jen-tse and Tu, Zhaopeng and Lyu, Michael R},
  journal={arXiv preprint arXiv:2310.12481},
  year={2023}
}
@article{li2024culture,
  title={Culture-gen: Revealing global cultural perception in language models through natural language prompting},
  author={Li, Huihan and Jiang, Liwei and Hwang, Jena D and Kim, Hyunwoo and Santy, Sebastin and Sorensen, Taylor and Lin, Bill Yuchen and Dziri, Nouha and Ren, Xiang and Choi, Yejin},
  journal={arXiv preprint arXiv:2404.10199},
  year={2024}
}
@inproceedings{alkhamissi-etal-2024-investigating,
    title = "Investigating Cultural Alignment of Large Language Models",
    author = "AlKhamissi, Badr  and
      ElNokrashy, Muhammad  and
      Alkhamissi, Mai  and
      Diab, Mona",
    booktitle = "Proceedings of the 62nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2024",
}
@inproceedings{naous-etal-2024-beer,
    title = "Having Beer after Prayer? Measuring Cultural Bias in Large Language Models",
    author = "Naous, Tarek  and
      Ryan, Michael J  and
      Ritter, Alan  and
      Xu, Wei",
    booktitle = "Proceedings of the 62nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    year = "2024",
}
@inproceedings{shen-etal-2024-understanding,
    title = "Understanding the Capabilities and Limitations of Large Language Models for Cultural Commonsense",
    author = "Shen, Siqi  and
      Logeswaran, Lajanugen  and
      Lee, Moontae  and
      Lee, Honglak  and
      Poria, Soujanya  and
      Mihalcea, Rada",
    booktitle = "Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers)",
    year = "2024",
}
@article{choenni2024self,
  title={Self-Alignment: Improving Alignment of Cultural Values in LLMs via In-Context Learning},
  author={Choenni, Rochelle and Shutova, Ekaterina},
  journal={arXiv preprint arXiv:2408.16482},
  year={2024}
}
@article{tao2024cultural,
  title={Cultural bias and cultural alignment of large language models},
  author={Tao, Yan and Viberg, Olga and Baker, Ryan S and Kizilcec, Ren{\'e} F},
  journal={PNAS nexus},
  volume={3},
  number={9},
  pages={pgae346},
  year={2024},
  publisher={Oxford University Press US}
}
@article{li2024culturellm,
  title={Culturellm: Incorporating cultural differences into large language models},
  author={Li, Cheng and Chen, Mengzhou and Wang, Jindong and Sitaram, Sunayana and Xie, Xing},
  journal={arXiv preprint arXiv:2402.10946},
  year={2024}
}
@misc{wvs,
      title={World Values Survey}, 
      author={World Values Survey},
      year={2022},
      howpublished={https://www.worldvaluessurvey.org/wvs.jsp}
}
@article{li2024culturepark,
  title={CulturePark: Boosting Cross-cultural Understanding in Large Language Models},
  author={Li, Cheng and Teney, Damien and Yang, Linyi and Wen, Qingsong and Xie, Xing and Wang, Jindong},
  journal={arXiv preprint arXiv:2405.15145},
  year={2024}
}
@article{feng2024modular,
  title={Modular pluralism: Pluralistic alignment via multi-llm collaboration},
  author={Feng, Shangbin and Sorensen, Taylor and Liu, Yuhan and Fisher, Jillian and Park, Chan Young and Choi, Yejin and Tsvetkov, Yulia},
  journal={arXiv preprint arXiv:2406.15951},
  year={2024}
}
@article{carver1982control,
  title={Control theory: A useful conceptual framework for personality--social, clinical, and health psychology.},
  author={Carver, Charles S and Scheier, Michael F},
  journal={Psychological bulletin},
  volume={92},
  number={1},
  pages={111},
  year={1982},
  publisher={American Psychological Association}
}
@article{sun2024benchmarking,
  title={Benchmarking Chinese Commonsense Reasoning of LLMs: From Chinese-Specifics to Reasoning-Memorization Correlations},
  author={Sun, Jiaxing and Huang, Weiquan and Wu, Jiang and Gu, Chenya and Li, Wei and Zhang, Songyang and Yan, Hang and He, Conghui},
  journal={arXiv preprint arXiv:2403.14112},
  year={2024}
}
@article{wang2023seaeval,
  title={SeaEval for multilingual foundation models: From cross-lingual alignment to cultural reasoning},
  author={Wang, Bin and Liu, Zhengyuan and Huang, Xin and Jiao, Fangkai and Ding, Yang and Aw, AiTi and Chen, Nancy F},
  journal={arXiv preprint arXiv:2309.04766},
  year={2023}
}
@article{mousi2024aradice,
  title={Aradice: Benchmarks for dialectal and cultural capabilities in llms},
  author={Mousi, Basel and Durrani, Nadir and Ahmad, Fatema and Hasan, Md Arid and Hasanain, Maram and Kabbani, Tameem and Dalvi, Fahim and Chowdhury, Shammur Absar and Alam, Firoj},
  journal={arXiv preprint arXiv:2409.11404},
  year={2024}
}
@article{putri2024can,
  title={Can LLM Generate Culturally Relevant Commonsense QA Data? Case Study in Indonesian and Sundanese},
  author={Putri, Rifki Afina and Haznitrama, Faiz Ghifari and Adhista, Dea and Oh, Alice},
  journal={arXiv preprint arXiv:2402.17302},
  year={2024}
}
@article{chiu2024culturalteaming,
  title={CulturalTeaming: AI-Assisted Interactive Red-Teaming for Challenging LLMs'(Lack of) Multicultural Knowledge},
  author={Chiu, Yu Ying and Jiang, Liwei and Antoniak, Maria and Park, Chan Young and Li, Shuyue Stella and Bhatia, Mehar and Ravi, Sahithya and Tsvetkov, Yulia and Shwartz, Vered and Choi, Yejin},
  journal={arXiv preprint arXiv:2404.06664},
  year={2024}
}
@article{huang2023large,
  title={Large language models cannot self-correct reasoning yet},
  author={Huang, Jie and Chen, Xinyun and Mishra, Swaroop and Zheng, Huaixiu Steven and Yu, Adams Wei and Song, Xinying and Zhou, Denny},
  journal={arXiv preprint arXiv:2310.01798},
  year={2023}
}
@article{kamoi2024can,
  title={When can llms actually correct their own mistakes? a critical survey of self-correction of llms},
  author={Kamoi, Ryo and Zhang, Yusen and Zhang, Nan and Han, Jiawei and Zhang, Rui},
  journal={Transactions of the Association for Computational Linguistics},
  volume={12},
  pages={1417--1440},
  year={2024},
  publisher={MIT Press 255 Main Street, 9th Floor, Cambridge, Massachusetts 02142, USA~…}
}
@article{gou2023critic,
  title={Critic: Large language models can self-correct with tool-interactive critiquing},
  author={Gou, Zhibin and Shao, Zhihong and Gong, Yeyun and Shen, Yelong and Yang, Yujiu and Duan, Nan and Chen, Weizhu},
  journal={arXiv preprint arXiv:2305.11738},
  year={2023}
}
@inproceedings{sun-etal-2024-critique,
    title = "The Critique of Critique",
    author = "Sun, Shichao  and
      Li, Junlong  and
      Yuan, Weizhe  and
      Yuan, Ruifeng  and
      Li, Wenjie  and
      Liu, Pengfei",
    booktitle = "Findings of the Association for Computational Linguistics: ACL 2024",
    year = "2024",
}
@article{rafailov2024direct,
  title={Direct preference optimization: Your language model is secretly a reward model},
  author={Rafailov, Rafael and Sharma, Archit and Mitchell, Eric and Manning, Christopher D and Ermon, Stefano and Finn, Chelsea},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}
@article{dubey2024llama,
  title={The llama 3 herd of models},
  author={Dubey, Abhimanyu and Jauhri, Abhinav and Pandey, Abhinav and Kadian, Abhishek and Al-Dahle, Ahmad and Letman, Aiesha and Mathur, Akhil and Schelten, Alan and Yang, Amy and Fan, Angela and others},
  journal={arXiv preprint arXiv:2407.21783},
  year={2024}
}
@article{yang2024qwen2,
  title={Qwen2. 5 technical report},
  author={Yang, An and Yang, Baosong and Zhang, Beichen and Hui, Binyuan and Zheng, Bo and Yu, Bowen and Li, Chengyuan and Liu, Dayiheng and Huang, Fei and Wei, Haoran and others},
  journal={arXiv preprint arXiv:2412.15115},
  year={2024}
}
@article{hurst2024gpt,
  title={Gpt-4o system card},
  author={Hurst, Aaron and Lerer, Adam and Goucher, Adam P and Perelman, Adam and Ramesh, Aditya and Clark, Aidan and Ostrow, AJ and Welihinda, Akila and Hayes, Alan and Radford, Alec and others},
  journal={arXiv preprint arXiv:2410.21276},
  year={2024}
}
@article{talmor2018commonsenseqa,
  title={Commonsenseqa: A question answering challenge targeting commonsense knowledge},
  author={Talmor, Alon and Herzig, Jonathan and Lourie, Nicholas and Berant, Jonathan},
  journal={arXiv preprint arXiv:1811.00937},
  year={2018}
}
@article{zellers2019hellaswag,
  title={Hellaswag: Can a machine really finish your sentence?},
  author={Zellers, Rowan and Holtzman, Ari and Bisk, Yonatan and Farhadi, Ali and Choi, Yejin},
  journal={arXiv preprint arXiv:1905.07830},
  year={2019}
}
@article{wang2024mmlu,
  title={Mmlu-pro: A more robust and challenging multi-task language understanding benchmark},
  author={Wang, Yubo and Ma, Xueguang and Zhang, Ge and Ni, Yuansheng and Chandra, Abhranil and Guo, Shiguang and Ren, Weiming and Arulraj, Aaran and He, Xuan and Jiang, Ziyan and others},
  journal={arXiv preprint arXiv:2406.01574},
  year={2024}
}
@article{hofstede2013vsm,
  title={VSM 2013},
  author={Hofstede, Geert and Minkov, Michael},
  journal={Values survey module},
  year={2013}
}
@article{ahn2024large,
  title={Large language models for mathematical reasoning: Progresses and challenges},
  author={Ahn, Janice and Verma, Rishu and Lou, Renze and Liu, Di and Zhang, Rui and Yin, Wenpeng},
  journal={arXiv preprint arXiv:2402.00157},
  year={2024}
}
@article{yuan2024self,
  title={Self-rewarding language models},
  author={Yuan, Weizhe and Pang, Richard Yuanzhe and Cho, Kyunghyun and Sukhbaatar, Sainbayar and Xu, Jing and Weston, Jason},
  journal={arXiv preprint arXiv:2401.10020},
  year={2024}
}
@article{bi2024deepseek,
  title={Deepseek llm: Scaling open-source language models with longtermism},
  author={Bi, Xiao and Chen, Deli and Chen, Guanting and Chen, Shanhuang and Dai, Damai and Deng, Chengqi and Ding, Honghui and Dong, Kai and Du, Qiushi and Fu, Zhe and others},
  journal={arXiv preprint arXiv:2401.02954},
  year={2024}
}
@article{pawar2024survey,
  title={Survey of cultural awareness in language models: Text and beyond},
  author={Pawar, Siddhesh and Park, Junyeong and Jin, Jiho and Arora, Arnav and Myung, Junho and Yadav, Srishti and Haznitrama, Faiz Ghifari and Song, Inhwa and Oh, Alice and Augenstein, Isabelle},
  journal={arXiv preprint arXiv:2411.00860},
  year={2024}
}
@article{hendrycks2020measuring,
  title={Measuring massive multitask language understanding},
  author={Hendrycks, Dan and Burns, Collin and Basart, Steven and Zou, Andy and Mazeika, Mantas and Song, Dawn and Steinhardt, Jacob},
  journal={arXiv preprint arXiv:2009.03300},
  year={2020}
}
@article{li2024attributing,
  title={Attributing culture-conditioned generations to pretraining corpora},
  author={Li, Huihan and Goel, Arnav and He, Keyu and Ren, Xiang},
  journal={arXiv preprint arXiv:2412.20760},
  year={2024}
}

==> tables/case_study.tex <==
\begin{table}
    \centering
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c}
    \toprule
    \textbf{Answer Type} & \textbf{Answer} & \textbf{Recall} & \textbf{F1} \\
    \midrule
    \model & \textbf{74.73} & \textbf{71.21} & \textbf{72.94} \\
    w/o Critique & 69.54 & 67.63 & 68.57\\
    w/o Multilingual & 70.95 & 70.63 & 70.79\\
    \bottomrule
    \end{tabular}
    }
    \caption{A case study on our GlobalCultureQA \data.}
    \label{tab:case_study}
\end{table}
